Investigations on ASIC for Triple-GEM Detectors

The main purpose of this work is to study the performance of the APV25 and VMM3a readout chips with regards to using them in the front-end readout system of a Triple-GEM detector. For the APV25, the Signal-to-Noise Ratio (SNR) was estimated with a cosmics measurement around 84.29 +/- 0.12. For the VMM3a, the noise of the chip was characterised in terms of the Equivalent Noise Charge (ENC) in the full parameter space and with increasing input capacitance. For the highest VMM gain and peaktime settings, the calculated ENC was about 300 electrons + 8 electrons/pF. Finally, a comparison was made between the two chips, based on their noise, while also the setup for future cosmics measurements with a VMM readout was prepared in order to also derive the VMM SNR ratio.

==> cover/Bachelor_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{ngerman}
    Bachelorarbeit in Physik\\
    angefertigt \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität\\
    Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
\lowertitleback{%
  \begin{otherlanguage}{ngerman}
    Ich versichere, dass ich diese Arbeit selbstständig
    verfasst und keine anderen als die angegebenen Quellen und
    Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Datum & Unterschrift
    \end{tabular}
  \end{otherlanguage}

  % \begin{otherlanguage}{UKenglish}
  %   I hereby declare that this thesis was formulated by
  %   myself and that no sources or tools other than those cited were used.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Date & Signature
  %   \end{tabular}
  % \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/Diplom_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the title page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\huge
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear
    }
  }
}


==> cover/Diplom_Final_Title.tex <==
%
% Title page layout for printed version
%
\titlehead{%
  \centering
  {\fontsize{44}{50}\selectfont
    Universität Bonn}

  \vspace*{20pt}

  \begin{singlespace}
    \fontsize{30}{40}\selectfont
    \InstituteName
  \end{singlespace}
}
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\vspace*{\fill}
  \raggedright
  {\normalsize
    \begin{otherlanguage}{ngerman}
      Dieser Forschungsbericht wurde als Diplomarbeit von der
      Mathematisch-Naturwissenschaftlichen Fakultät der Universität Bonn
      angenommen.
    \end{otherlanguage}

    \vspace*{10ex minus 4ex}

    \noindent
    \begin{tabular}{@{}ll}
      Angenommen am:         & \thesissubmit\\
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  }
}

\maketitle


==> cover/Diplom_Submit_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{ngerman}
    Diplomarbeit in Physik\\
    angefertigt \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität\\
    Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
\lowertitleback{%
  \begin{otherlanguage}{ngerman}
    Ich versichere, dass ich diese Arbeit selbstständig
    verfasst und keine anderen als die angegebenen Quellen und
    Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Datum & Unterschrift
    \end{tabular}
  \end{otherlanguage}

  % \begin{otherlanguage}{UKenglish}
  %   I hereby declare that this thesis was formulated by
  %   myself and that no sources or tools other than those cited were used.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Date & Signature
  %   \end{tabular}
  % \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/Guide_Submit_Title.tex <==
% chktex-file 21

% Title page layout for submitted version.
\title{\thesistitle}
\subtitle{\vspace*{4ex}
  \begin{otherlanguage}{ngerman}
    Hinweise und Tipps\\
    zur\\
    Produktion einer Bachelor/Master/Doktorarbeit\\
    in der\\
    Mathematisch-Naturwissenschaftlichen-Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
}
\author{%
  vorgelegt von\\
  \thesisauthor\\
  aus\\
  \thesistown%
}
\date{Version \guideversion\\
  \today}
\publishers{%
  Bonn \thesisyear%
}
\lowertitleback{%
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo\\[2ex]
      Tag der Promotion: & \\
      Erscheinungsjahr: & 
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/Master_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the title page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\huge
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear
    }
  }
}


==> cover/Master_Final_Title.tex <==
%
% Title page layout for printed version
%
\titlehead{%
  \centering
  {\fontsize{44}{50}\selectfont
    Universität Bonn}

  \vspace*{20pt}

  \begin{singlespace}
    \fontsize{30}{40}\selectfont
    \InstituteName
  \end{singlespace}
}
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\vspace*{\fill}
  \raggedright
  {\normalsize
    \begin{otherlanguage}{ngerman}
      Dieser Forschungsbericht wurde als Masterarbeit von der
      Mathematisch-Naturwissenschaftlichen Fakultät der Universität Bonn
      angenommen.
    \end{otherlanguage}

    \vspace*{10ex minus 4ex}

    \noindent
    \begin{tabular}{@{}ll}
      Angenommen am:         & \thesissubmit\\
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  }
}

\maketitle


==> cover/Master_Submit_Title.tex <==
%
% Title page layout for submitted version
%
\title{\thesistitle}
\author{\LARGE\thesisauthor}
\date{}
\publishers{\LARGE
  \begin{otherlanguage}{UKenglish}
    Masterarbeit in Physik\\
    angefertigt im \inInstitute\\[3ex]
    vorgelegt der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Universität Bonn\\[3ex]
    \thesismonth{} \thesisyear
  \end{otherlanguage}
  \vspace*{\fill}
}
%Dieser Forschungsbericht wurde als Masterarbeit von derMathematisch-Naturwissenschaftlichen Fakultät der Universität Bonn angenommen.
\lowertitleback{%
  % \begin{otherlanguage}{ngerman}
  %   Ich versichere, dass ich diese Arbeit selbstständig
  %   verfasst und keine anderen als die angegebenen Quellen und
  %   Hilfsmittel benutzt sowie die Zitate kenntlich gemacht habe.

  %   \vspace*{4ex minus 0.5ex}

  %   \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
  %     Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
  %     & Datum & Unterschrift
  %   \end{tabular}
  % \end{otherlanguage}

  \begin{otherlanguage}{UKenglish}
    I hereby declare that this thesis was formulated by
    myself and that no sources or tools other than those cited were used.

    \vspace*{4ex minus 0.5ex}

    \begin{tabular}{@{}lc@{\hspace*{4.0cm}}c}
      Bonn, &  \makebox[3cm]{\dotfill} & \makebox[6cm]{\dotfill}\\
      & Date & Signature
    \end{tabular}
  \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/PhD_Cover.tex <==
%
% Cover page layout for the department library version
%
% Make the top margin on the cover page larger and also increase the
% size of the left margin to allow for binding. These parameters may
% have to be adjusted if you change the fraction of the page area that
% is used for the text.
% Changing margins works well. Changing the text height has a bad
% effect on the table of contents.
%
{\thispagestyle{empty}
  \addtolength{\oddsidemargin}{1.0cm}\addtolength{\topmargin}{1.0cm}
  \rmfamily\setlength{\parindent}{0pt}
  \begin{center}
    {\fontsize{44}{50}\selectfont
      Universität Bonn}

    \vspace*{20pt}

    \begin{singlespace}
      \fontsize{30}{40}\selectfont
      \InstituteName
    \end{singlespace}

    \vspace*{40pt}

    \begin{onehalfspace}
      \bfseries\huge
      \thesistitle
    \end{onehalfspace}

    \vspace*{20pt}

    {\LARGE
      \thesisauthor
    }
  \end{center}

  \vspace*{\fill}

  \thesisabstract

  \vspace*{\fill}

  {\normalfont\normalsize
    \parbox{0.3\textwidth}{\InstituteAddress}
    \parbox{0.4\textwidth}{%
      \centering
      \includegraphics[width=5cm]{instituts_siegel}
    }
    \parbox{0.3\textwidth}{%
      \thesisnumber\\
      \thesismonth{} \thesisyear\\
      ISSN-0172-8741
    }
  }
}


==> cover/PhD_Final_Title.tex <==
%
% Title page layout for published version
%
% \titlehead{%
%   \centering
%   {\fontsize{44}{50}\selectfont
%     Universität Bonn}

%   \vspace*{20pt}

%   \begin{singlespace}
%     \fontsize{30}{40}\selectfont
%     \InstituteName
%   \end{singlespace}
% }
\title{\thesistitle}
\subtitle{\vspace*{4ex}
  \begin{otherlanguage}{ngerman}
    Dissertation\\
    zur\\
    Erlangung des Doktorgrades (Dr.\ rer.\ nat.)\\
    der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
}
\author{%
  von\\
  \LARGE \thesisauthor\\
  aus\\
  \thesistown
}
\date{}
\publishers{%
  Bonn, \thesissubmit
}
\lowertitleback{\normalsize
  \raggedright
  \begin{otherlanguage}{ngerman}
    Angefertigt mit Genehmigung der Mathematisch-Naturwissenschaftlichen Fakultät der Rheinischen Friedrich-Wilhelms-Universität Bonn
    % Dieser Forschungsbericht wurde als Dissertation von der
    % Mathematisch-Naturwissenschaftlichen Fakultät der Universität
    % Bonn angenommen und ist auf dem
    % Hochschulschriftenserver der ULB Bonn
    % \url{http://hss.ulb.uni-bonn.de/diss_online} elektronisch
    % publiziert.
  \end{otherlanguage}

  \vspace*{10ex minus 4ex}

  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo\\[2ex]
      Tag der Promotion: & \thesispromotion\\
      Erscheinungsjahr: & \thesisyear
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> cover/PhD_Submit_Title.tex <==
%
% Title page layout for submitted version.
%
\title{\thesistitle}
\subtitle{\vspace*{4ex}
  \begin{otherlanguage}{ngerman}
    Dissertation\\
    zur\\
    Erlangung des Doktorgrades (Dr.\ rer.\ nat.)\\
    der\\
    Mathematisch-Naturwissenschaftlichen Fakultät\\
    der\\
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
}
\author{%
  vorgelegt von\\
  \thesisauthor\\
  aus\\
  \thesistown
}
\date{}
\publishers{%
  Bonn \thesisyear
}
\lowertitleback{\normalsize
  \begin{otherlanguage}{ngerman}
    Angefertigt mit Genehmigung der 
    Mathematisch-Naturwissenschaftlichen Fakultät der
    Rheinischen Friedrich-Wilhelms-Universität Bonn
  \end{otherlanguage}
  
  \vspace*{10ex minus 4ex}
  
  \noindent
  \begin{otherlanguage}{ngerman}
    \begin{tabular}{@{}ll}
      \thesisrefereeonetext: & \thesisrefereeone\\
      \thesisrefereetwotext: & \thesisrefereetwo\\[2ex]
      Tag der Promotion:      & \\
      Erscheinungsjahr:       & 
    \end{tabular}
  \end{otherlanguage}
}

\maketitle


==> thesis_cv.tex <==
\definecolor{lightgray}{gray}{0.8}
\newcolumntype{L}{>{\raggedleft}p{0.15\textwidth}}
\newcolumntype{R}{p{0.8\textwidth}}
\newcommand\VRule{\color{lightgray}\vrule width 0.5pt}

\thispagestyle{empty}
\section*{Curriculum Vitae}

\subsection*{Personal Details}

\begin{tabular}{L!{\VRule}R}
Name & Johann Schmidt \\
Date of Birth &  \\
Email & abc@physik.uni-def.de \\
Family status & Single
\end{tabular}

\subsection*{Education}

\begin{tabular}{L!{\VRule}R}
1997--2003 & Abitur, ABC Secondary School, Hamburg, Germany\\
2004--2007 & BSc in Physics, Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany.\\
2006 & CERN Summer Student, Geneva, Switzerland. \\
2007--2009 &  MSc in Physics Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany. \\
2009--2012 &  PhD in Physics, Rheinische Friedrich-Wilhelms-Universität, Bonn, Germany. \\
2012 & Advanced Data Analysis School, Frankfurt, Germany.
\end{tabular}

\subsection*{Professional Experience}

\begin{tabular}{L!{\VRule}R}
2004 & Summer Student at CERN, Geneva, Switzerland. \\
2007--2012 & Doctoral work at the University of Bonn, Germany. \\
2008--2009 & Fieldwork at CERN, Geneva, Switzerland.\\
2011 & Talk at the Advanced Physics Conference, Timbucto
\end{tabular}

\subsection*{Languages}
\begin{tabular}{L!{\VRule}R}
German & Mother tongue \\
English & Fluent \\
Russian & Basic
\end{tabular}

